Theoretical Modelling of Gamma-Ray Burst 090510

Gamma-ray bursts detected at high energies provide valuable insights into the emission mechanisms behind these still puzzling enigmatic events. In this study, we focus on GRB 090510, which is an unusual short GRB exhibiting plateau emission observed by the Fermi-LAT. Using the general relativistic magnetohydrodynamic code (HARM), we aim to infer the key properties of this GRB, such as the jet opening angle, the energetics, the Lorentz Gamma factor, the jet structure and its variability, and the progenitor parameters of the compact binary system. We explored both the 2D and 3D models and estimated the variability timescales. Our findings show that the predicted jet opening angle is within $88\%$ of the observed upper limit from observations, and the energetics are in general agreement with observed values when accounting for the evolution of jet opening angle with redshift. This work establishes the foundation for ongoing exploration, which will further align the theoretical model simulations with observational data.

==> organizers.tex <==
%to switch ON running title
%\markboth{Organizing committees}{Organizing committees}

\wstoc{Organizing committees}{}

\title{Organizing committees}

\begin{center}
{\bf Series editorial board}\\
{\it for the series on advances in quantum many-body theory}
\end{center}
\vspace*{1em}

\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
C. E. Campbell & -- University of Minnesota, USA \\
J. W. Clark & -- Washington University, St.\ Louis, USA \\
S. Fantoni & -- SISSA, Trieste, Italy
\end{tabular}

\vspace*{0.12in}

\noindent
\begin{center}
{\bf International advisory committee}\\
{\it for the Series of International Conferences on}\\
{\it Recent Progress in Many-Body Theories}
\end{center}
\vspace*{1em}

\noindent
\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
S. Fantoni (Secretary) & -- SISSA, Trieste, Italy\\
C. E. Campbell (Treasurer) & -- University of Minnesota, USA\\
H. K\"{u}mmel (Hon.\ President) & -- Ruhr-Universit\"{a}t
Bochum, Germany \\
J. A. Carlson & -- Los Alamos National Laboratory, USA \\
S. A. Chin & -- Texas A \& M University, USA \\
J. W. Clark & -- Washington University, St.~Louis, USA \\
P. Fulde & -- Max-Planck-Institut f\"{u}r Komplexer  \\
& ~~~Systeme, Dresden, Germany\\
A. Kallio & -- University of Oulu, Finland \\
E. Krotscheck & -- Johannes Universit\"{a}t Linz, Austria \\
C. Lhuillier & -- Universit\'{e} Pierre et Marie Curie, Paris\\
A. MacDonald & -- Indiana University, Bloomington, USA \\
E. Manousakis & -- Florida State University, USA \\
D. Neilson & -- University of New South Wales, Sydney, \\
& ~~~Australia \\
M. L. Ristig & -- Universit\"{a}t zu K\"{o}ln, Germany
\end{tabular}


==> preface.tex <==
%to switch ON running title
%\markboth{Preface}{Preface}

\wstoc{Preface}{}

\title{Preface}

The {\it Tenth International Conference on Recent Progress in
Many-Body Theories} (RPMBT-10) was held at the University of
Washington in Seattle, USA during the period 10-15 September, 1999.
The present volume contains the texts of most of the invited talks
delivered at the conference and a selection from among the many poster
presentations.

The general format and style of the conference followed the accepted
and well-developed pattern for the series, focusing on the
development, refinement and important applications of the techniques
of quantum many-body theory.  The intention of the series has always
been to cover in a broad and balanced fashion both the entire spectrum
of theoretical tools developed to tackle the quantum many-body problem
and their major fields of application.  One of the main aims of the
series is to foster the exchange of ideas and techniques among
physicists working in such diverse areas of applications of many-body
techniques as nuclear and subnuclear physics, astrophysics, atomic and
molecular physics, quantum chemistry, complex systems, quantum field
theory, strongly correlated electronic systems, magnetism, quantum
fluids and condensed matter physics.

Quantum many-body theory as a discipline in its own right dates
largely from the 1950's, and is hence in many senses already a
mature subject.  Despite this apparent maturity the field remains
vibrant and active, vigorous and exciting, vital and important.
Indeed, the successes, importance and vitality of the field have
very clearly been recognized by the sharing of the 1998 Nobel Prizes
in both Physics and Chemistry by the many-body theorists Robert
Laughlin, Walter Kohn and John Pople.  It is a source of great
pleasure to all of us who work in quantum many-body theory that
important achievements in our subject have been thus recognized at
the very highest level.  We were also especially delighted that two
of these then most recent Nobel Laureates, Kohn and Laughlin,
accepted invitations to deliver keynote lectures at RPMBT-10...

A major challenge will be to define and explore these important
areas of overlap in such likely arenas as phase transitions and the
related competing effects of quantum versus thermal fluctuations;
spontaneous symmetry breaking; the unifying role of gauge invariance
(and perhaps other symmetries); concepts from complexity theory,
including the role of correlations and fluctuations in complex
systems, and the competition between analysis and synthesis as modes
of understanding many-body systems; entropy and its generation and
flow; and nonlinearity and its appearance and role at the boundary
between microscopic and mesoscopic descriptions of many-body
systems.  One can perhaps begin to glimpse some insights within the
present proceedings into some of these as areas of future forefront
activity in quantum many-body theory. In this case it may well be
that RPMBT-10 and its immediate successors will later be identified
as the first in the series at which the seeds of the new discourse
between quantum many-body/field theory and statistical physics took
root.

In any event, the Local Organizing and Programme Committees deserve
great thanks in creating a well-run and productive meeting, with an
exciting programme of talks and poster presentations. It is a pleasure
to thank all of them for their hard work, especially Aurel Bulgac who,
as Chairman, has led and guided them throughout.

\vspace*{0.35in}

\noindent
R.F. Bishop \hfill Manchester, U.K.\\
{\itshape (Chairman, International Advisory Committee}
\hfill 31 December 1999\\
{\itshape for the Series of International Conferences on}\\
{\itshape Recent Progress in Many-Body Theories)}

